Control of the Vertical Gradient Freeze crystal growth process via backstepping

This contribution presents a backstepping-based state feedback design for the tracking control of a two-phase Stefan problem which is encountered in the Vertical Gradient Freeze crystal growth process. A two-phase Stefan problem consists of two coupled free boundary problems and is a vital part of many crystal growth processes due to the time-varying extent of crystal and melt during growth. In addition, a different approach for the numerical approximation of the backstepping transformations kernel is presented.

==> acknowledgements.tex <==
\begin{ack}
This work has been funded by the Deutsche Forschungsgemeinschaft (DFG) 
[project number WI 4412/1-1%, FR 3671/1-1
].
\end{ack}

